Risks of heterogeneously persistent higher moments

Using intraday data for the cross-section of individual stocks, we show that both transitory and persistent fluctuations in realized market and average idiosyncratic volatility, skewness and kurtosis are differentially priced in the cross-section of asset returns, implying a heterogeneous persistence structure of different sources of higher moment risks. Specifically, we find that idiosyncratic transitory shocks to volatility as well as idiosyncratic persistent shocks to skewness contain strong commonalities that are relevant to investors.

==> Tables/crsp3m1usd.tex <==
\begin{tabular}{l c c c c c c }
\hline
\hline
\textbf{Variable} & \textbf{1} & \textbf{2} & \textbf{3} & \textbf{4} & \textbf{5} & \textbf{6} \\
\hline
const & 0.000266 & 0.000293 & 0.000336 & 0.000261 & 0.000297 & 0.000333 \\  & (1.841497) & (2.088281) & (2.623671) & (1.841913) & (2.124197) & (2.608281) \\
$RVOL_{t}^{(m)}$ & -6.2e-05 &  & -5.7e-05 &  &  &  \\  & (-1.502881) &  & (-1.543698) &  &  &  \\
$RS_{t}^{(m)}$ & -0.005059 &  & -0.003569 &  &  &  \\  & (-0.706861) &  & (-0.676031) &  &  &  \\
$RK_{t}^{(m)}$ & -0.003795 &  & 0.002053 &  &  &  \\  & (-0.226942) &  & (0.148953) &  &  &  \\
$RVOL_{t}^{(m, \tr)}$ &  &  &  & -5.3e-05 &  & -4.2e-05 \\  &  &  &  & (-1.270376) &  & (-1.092463) \\
$RVOL_{t}^{(m, \p)}$ &  &  &  & -4e-06 &  & -4e-06 \\  &  &  &  & (-0.540742) &  & (-0.689164) \\
$RS_{t}^{(m, \tr)}$ &  &  &  & -0.005507 &  & -0.004293 \\  &  &  &  & (-0.807545) &  & (-0.850716) \\
$RS_{t}^{(m, \p)}$ &  &  &  & -4.5e-05 &  & -7.7e-05 \\  &  &  &  & (-0.375625) &  & (-0.719172) \\
$RK_{t}^{(m, \tr)}$ &  &  &  & -0.006475 &  & 0.002166 \\  &  &  &  & (-0.422686) &  & (0.165463) \\
$RK_{t}^{(m, \p)}$ &  &  &  & -0.000965 &  & -0.000738 \\  &  &  &  & (-0.948218) &  & (-0.813079) \\
$RVOL_{t}^{(I)}$ &  & -8.5e-05 & -9.3e-05 &  &  &  \\  &  & (-1.531039) & (-1.635753) &  &  &  \\
$RS_{t}^{(I)}$ &  & -0.001853 & -0.001206 &  &  &  \\  &  & (-0.81492) & (-0.685896) &  &  &  \\
$RK_{t}^{(I)}$ &  & -0.005946 & -0.002021 &  &  &  \\  &  & (-1.364476) & (-0.569856) &  &  &  \\
$RVOL_{t}^{(I, \tr)}$ &  &  &  &  & -0.000115 & -8.8e-05 \\  &  &  &  &  & (-1.934482) & (-1.505646) \\
$RVOL_{t}^{(I, \p)}$ &  &  &  &  & 8e-06 & 1e-06 \\  &  &  &  &  & (0.516714) & (0.068466) \\
$RS_{t}^{(I, \tr)}$ &  &  &  &  & -0.001638 & -0.001254 \\  &  &  &  &  & (-0.741913) & (-0.74011) \\
$RS_{t}^{(I, \p)}$ &  &  &  &  & -8.3e-05 & -6.3e-05 \\  &  &  &  &  & (-1.692773) & (-1.350828) \\
$RK_{t}^{(I, \tr)}$ &  &  &  &  & -0.004646 & -0.001672 \\  &  &  &  &  & (-1.125943) & (-0.514135) \\
$RK_{t}^{(I, \p)}$ &  &  &  &  & -0.000449 & -4e-04 \\  &  &  &  &  & (-0.801284) & (-0.761161) \\
MKT &  &  & -0.00809 &  &  & -0.008008 \\  &  &  & (-0.869131) &  &  & (-0.867598) \\
SMB &  &  & -0.000653 &  &  & -0.001724 \\  &  &  & (-0.16593) &  &  & (-0.439589) \\
HML &  &  & 0.010806 &  &  & 0.011903 \\  &  &  & (1.580461) &  &  & (1.740304) \\
\hline
\end{tabular}


==> Tables/crsp3m5usd.tex <==
\begin{tabular}{l c c c c c c }
\hline
\hline
\textbf{Variable} & \textbf{1} & \textbf{2} & \textbf{3} & \textbf{4} & \textbf{5} & \textbf{6} \\
\hline
const & 0.000194 & 0.000217 & 0.000263 & 0.00021 & 0.00024 & 0.000272 \\  & (1.634817) & (1.893592) & (2.684692) & (1.802089) & (2.100192) & (2.74054) \\
$RVOL_{t}^{(m)}$ & -5.5e-05 &  & -4.2e-05 &  &  &  \\  & (-1.195889) &  & (-1.054257) &  &  &  \\
$RS_{t}^{(m)}$ & -0.002566 &  & -0.001861 &  &  &  \\  & (-0.312813) &  & (-0.332151) &  &  &  \\
$RK_{t}^{(m)}$ & -0.016712 &  & -0.005314 &  &  &  \\  & (-0.884968) &  & (-0.368476) &  &  &  \\
$RVOL_{t}^{(m, \tr)}$ &  &  &  & -5.2e-05 &  & -3.7e-05 \\  &  &  &  & (-1.112225) &  & (-0.937916) \\
$RVOL_{t}^{(m, \p)}$ &  &  &  & 1e-06 &  & 0 \\  &  &  &  & (0.108501) &  & (0.040387) \\
$RS_{t}^{(m, \tr)}$ &  &  &  & -0.003449 &  & -0.002728 \\  &  &  &  & (-0.447558) &  & (-0.508721) \\
$RS_{t}^{(m, \p)}$ &  &  &  & 6.3e-05 &  & -7e-06 \\  &  &  &  & (0.574991) &  & (-0.080784) \\
$RK_{t}^{(m, \tr)}$ &  &  &  & -0.019541 &  & -0.006327 \\  &  &  &  & (-1.1318) &  & (-0.459669) \\
$RK_{t}^{(m, \p)}$ &  &  &  & -0.001122 &  & -0.000946 \\  &  &  &  & (-1.045697) &  & (-1.052204) \\
$RVOL_{t}^{(I)}$ &  & -9.2e-05 & -9.9e-05 &  &  &  \\  &  & (-1.432108) & (-1.609138) &  &  &  \\
$RS_{t}^{(I)}$ &  & -0.001345 & -0.001112 &  &  &  \\  &  & (-0.518896) & (-0.563769) &  &  &  \\
$RK_{t}^{(I)}$ &  & -0.007643 & -0.00456 &  &  &  \\  &  & (-1.550091) & (-1.197879) &  &  &  \\
$RVOL_{t}^{(I, \tr)}$ &  &  &  &  & -0.00013 & -9.9e-05 \\  &  &  &  &  & (-1.836677) & (-1.534636) \\
$RVOL_{t}^{(I, \p)}$ &  &  &  &  & 7e-06 & -2e-06 \\  &  &  &  &  & (0.452278) & (-0.104328) \\
$RS_{t}^{(I, \tr)}$ &  &  &  &  & -0.001172 & -0.001223 \\  &  &  &  &  & (-0.467577) & (-0.647101) \\
$RS_{t}^{(I, \p)}$ &  &  &  &  & -6.2e-05 & -4.8e-05 \\  &  &  &  &  & (-1.16309) & (-0.952065) \\
$RK_{t}^{(I, \tr)}$ &  &  &  &  & -0.006736 & -0.003885 \\  &  &  &  &  & (-1.457735) & (-1.086416) \\
$RK_{t}^{(I, \p)}$ &  &  &  &  & -0.000524 & -0.000496 \\  &  &  &  &  & (-0.957011) & (-0.973961) \\
MKT &  &  & -0.007259 &  &  & -0.007606 \\  &  &  & (-0.702027) &  &  & (-0.747095) \\
SMB &  &  & -0.000159 &  &  & -0.001232 \\  &  &  & (-0.037617) &  &  & (-0.29442) \\
HML &  &  & 0.01092 &  &  & 0.011902 \\  &  &  & (1.476544) &  &  & (1.618948) \\
\hline
\end{tabular}


==> Tables/spdaily.tex <==
\begin{tabular}{l c c c c c c }
\hline
\hline
& \multicolumn{3}{c}{Panel A: Aggregate} & \multicolumn{3}{c}{Panel B: Heterogeneous} \\  
\cline{2-7}
\textbf{Variable} & \textbf{1} & \textbf{2} & \textbf{3} & \textbf{4} & \textbf{5} & \textbf{6} \\
\hline
$RVOL_{t}^{(m)}$ & -0.000122 &  &  &  & -0.000109 &  \\  & (-1.607513) &  &  &  & (-1.671282) &  \\
$RS_{t}^{(m)}$ & -0.005618 &  &  &  & 1e-06 &  \\  & (-0.54389) &  &  &  & (9.9e-05) &  \\
$RK_{t}^{(m)}$ & 0.004954 &  &  &  & 0.013684 &  \\  & (0.194747) &  &  &  & (0.661035) &  \\
$RVOL_{t}^{(m, \tr)}$ &  & -0.000151 &  &  &  & -0.000114 \\  &  & (-2.048782) &  &  &  & (-1.903472) \\
$RVOL_{t}^{(m, \p)}$ &  & 1.9e-05 &  &  &  & 1e-05 \\  &  & (0.812579) &  &  &  & (0.585774) \\
$RS_{t}^{(m, \tr)}$ &  & -0.003684 &  &  &  & -0.000484 \\  &  & (-0.387517) &  &  &  & (-0.073113) \\
$RS_{t}^{(m, \p)}$ &  & 0.000193 &  &  &  & -6e-06 \\  &  & (0.610221) &  &  &  & (-0.02153) \\
$RK_{t}^{(m, \tr)}$ &  & -0.003663 &  &  &  & 0.010798 \\  &  & (-0.16252) &  &  &  & (0.57424) \\
$RK_{t}^{(m, \p)}$ &  & -0.001516 &  &  &  & -0.002113 \\  &  & (-0.59466) &  &  &  & (-1.017173) \\
$RVOL_{t}^{(I)}$ &  &  & -0.000205 &  & -0.000218 &  \\  &  &  & (-1.920634) &  & (-2.140096) &  \\
$RS_{t}^{(I)}$ &  &  & -0.002449 &  & -0.000654 &  \\  &  &  & (-0.743312) &  & (-0.262662) &  \\
$RK_{t}^{(I)}$ &  &  & -0.003375 &  & 0.001592 &  \\  &  &  & (-0.535446) &  & (0.313313) &  \\
$RVOL_{t}^{(I, \tr)}$ &  &  &  & -0.000208 &  & -0.000182 \\  &  &  &  & (-2.127537) &  & (-1.937156) \\
$RVOL_{t}^{(I, \p)}$ &  &  &  & -1.3e-05 &  & -2.8e-05 \\  &  &  &  & (-0.312878) &  & (-0.847539) \\
$RS_{t}^{(I, \tr)}$ &  &  &  & -0.002531 &  & -0.000921 \\  &  &  &  & (-0.803988) &  & (-0.384026) \\
$RS_{t}^{(I, \p)}$ &  &  &  & -0.000128 &  & -8.7e-05 \\  &  &  &  & (-1.342432) &  & (-1.009159) \\
$RK_{t}^{(I, \tr)}$ &  &  &  & -0.004492 &  & 0.000393 \\  &  &  &  & (-0.780878) &  & (0.081852) \\
$RK_{t}^{(I, \p)}$ &  &  &  & 0.000477 &  & 0.001045 \\  &  &  &  & (0.537538) &  & (1.346655) \\
%MKT &  &  &  &  & -0.006373 & -0.00707 \\  &  &  &  &  & (-0.540654) & (-0.606209) \\
%SMB &  &  &  &  & 0.002318 & 0.001807 \\  &  &  &  &  & (0.460144) & (0.3642) \\
%HML &  &  &  &  & 0.010046 & 0.010228 \\  &  &  &  &  & (1.230135) & (1.253548) \\
\hline\hline
\end{tabular}

